Channel-Aware Domain-Adaptive Generative Adversarial Network for Robust Speech Recognition

While pre-trained automatic speech recognition (ASR) systems demonstrate impressive performance on matched domains, their performance often degrades when confronted with channel mismatch stemming from unseen recording environments and conditions. To mitigate this issue, we propose a novel channel-aware data simulation method for robust ASR training. Our method harnesses the synergistic power of channel-extractive techniques and generative adversarial networks (GANs). We first train a channel encoder capable of extracting embeddings from arbitrary audio. On top of this, channel embeddings are extracted using a minimal amount of target-domain data and used to guide a GAN-based speech synthesizer. This synthesizer generates speech that faithfully preserves the phonetic content of the input while mimicking the channel characteristics of the target domain. We evaluate our method on the challenging Hakka Across Taiwan (HAT) and Taiwanese Across Taiwan (TAT) corpora, achieving relative character error rate (CER) reductions of 20.02% and 9.64%, respectively, compared to the baselines. These results highlight the efficacy of our channel-aware data simulation method for bridging the gap between source- and target-domain acoustics.

==> rebuttal.tex <==
The authors would like to thank the anonymous reviewers for their positive comments on the technical novelty and writing of this paper. Below are responses to the major issues raised by the reviewers.

\subsection{Responses to Reviewer #1:}
\textbf{Questions: Experiments based on the challenging Hakka Across Taiwan (HAT) and Taiwanese Across Taiwan (TAT) corpora demonstrated the effectiveness of proposed CADA-GAN. But the target domain is one or specific case, which might limit the application of fine-tuned model. Moreover, GAN training is generally unstable.}
Answers: Thank you for your insightful comments. We recognize the limitation of focusing solely on the HAT and TAT corpora and agree that evaluating CADA-GAN on more diverse datasets is essential to demonstrate its generalizability and robustness. Expanding the scope of evaluation is a key goal for our future work. Regarding the stability of GAN training, we acknowledge this challenge and have incorporated specific techniques to mitigate instability in our training process. While the results on the current target domain are promising, we will continue to refine our approach and validate its performance across multiple domains to ensure broader applicability.
 
\subsection{Responses to Reviewer #2:}
\textbf{Question: However, the paper could benefit from a better reference section.}
Answers: Thank you for your valuable feedback. We agree that the reference section can be further strengthened and will incorporate more recent and relevant works, particularly those focusing on GAN-based speech synthesis and channel compensation. This improvement will be addressed in the next revised version of the paper.
 
\subsection{Responses to Reviewer #3:}
\textbf{Question: The channel encoder used is pre-trained on HAT corpus; it is advisable to test a different encoder to ensure there is no data leakage.}
Answers: We appreciate your thoughtful input. While the HAT and TAT datasets share overlapping channel names, there is no evidence suggesting they were recorded using the same types or brands of devices. However, to mitigate any risk of data leakage, we will prioritize testing on additional, more diverse datasets in future work. Exploring alternative channel encoders will also be a key step to further validate the robustness and generalizability of our framework.
